Reward-rational (implicit) choice: A unifying formalism for reward learning

It is often difficult to hand-specify what the correct reward function is for a task, so researchers have instead aimed to learn reward functions from human behavior or feedback. The types of behavior interpreted as evidence of the reward function have expanded greatly in recent years. We've gone from demonstrations, to comparisons, to reading into the information leaked when the human is pushing the robot away or turning it off. And surely, there is more to come. How will a robot make sense of all these diverse types of behavior? Our key insight is that different types of behavior can be interpreted in a single unifying formalism - as a reward-rational choice that the human is making, often implicitly. The formalism offers both a unifying lens with which to view past work, as well as a recipe for interpreting new sources of information that are yet to be uncovered. We provide two examples to showcase this: interpreting a new feedback type, and reading into how the choice of feedback itself leaks information about the reward.

==> composing_fdbk.tex <==
\section{Looking forward:  new behavior types}  \label{sec:unstr-compos}

The types of feedback or behavior we have discussed so far are by no means the only types possible. New ones will inevitably be invented. But when designing a new type of feedback, it is often difficult to understand what the relationship is between the reward $\reward$ and the feedback $\fdbkch$. Reward-rational choice suggests a recipe for uncovering this link -- define what the implicit set of options the human is choosing from is, and how those options ground to trajectories. Then, Equation \ref{eq:rat-choice2} provides a formal model for the human feedback.

To illustrate the utility of this, we identify two new types in this section. We start with hypothesizing another type of direct feedback that a robot could ask a human for, which we call \emph{credit assignment}. We then move onto an indirect source of information that we identified as a direct consequence of applying the formalism to \emph{combine} feedback types.

\subsection{A simple starting example} \label{sec:new-fbdk}
We first provide a quick example of a new (hypothetical) type of feedback, which we call credit assignment. Given a trajectory $\traj_R$ of length $T$, the human is asked to pick a segment of length $k < T$ that has maximal reward. We doubt the set of choices in an implementation of credit assignment would be explicit, however the implicit set of choices $\choices$ is then the set of all segments of length $k$. The grounding function $\map$ is simply the identity. With this choice of $\choices$ and $\map$ in hand, the human can now be modeled according to Equation \ref{eq:rat-choice2}, as we show in the last rows of Tables \ref{tab:c-grding} and \ref{tab:policies}.

While we do not argue that our formalism will apply to \emph{all} types of feedback, we believe that it applies to \emph{many}, even to types that initially seem to have a more obvious, literal interpretation (e.g. reward and punishment, Section \ref{sec:applying-formalism}).%


\subsection{Meta-choice: a new source of information}\label{sec:hierc-compos} 


So far we have talked about learning from individual types of behaviors. But we do not want our robots stuck with a single type: we want them to 1) read into all the leaked information, and 2) learn from all the purposeful feedback.
Luckily, the reward-rational choice framework also guides us in formalizing combinations of behavior.

In what follows, we start with a naive way of combining feedback types: treat each individual feedback received as a reward rational choice, and update the robot's belief. We then move to make the observation that the moment we open it up to multiple types of feedback, the person is not stuck with a single type and is actually choosing which type to use. \emph{We propose that this itself is a reward-rational implicit choice, and therefore leaks information about the reward.}

\noindent\textbf{Naive: conditional independence given reward.} Suppose we observe multiple types of behavior from a human. For example, we might have received a demonstration from a human during training, and then a correction during deployment, which was followed by the human prematurely switching the robot off. The observational model in (\ref{eq:rat-choice-det}) for a single type of behavior also provides a natural way to model combinations of behavior. If each observation is conditionally independent given the reward, then according to (\ref{eq:rat-choice-det}), the probability of observing a vector $\mathbf{\fdbk}$ of $n$ behavioral signals (of possibly different types) is equal to
\begin{align} \label{eq:prob-combine}
    \pr(\mathbf{\fdbk} \mid r) = \prod_i \frac{\exp(\rat \cdot \reward (\map_i(\mathbf{\fdbk}_i)))}{\sum_{\fdbk \in \choices_i} \exp(\rat \cdot \reward (\map_i(\fdbk)))} \,.
\end{align}
Given this likelihood function for the human's behavior, the robot can infer the reward function using the approaches and approximations described in \sref{sec:robot-inf}. Recent work has often focused on combining specific types of behavior, such as trajectory comparisons and demonstrations \citep{ibarz2018reward,palan2019learning}. We note that the formulation in (\ref{eq:prob-combine}) is general and applies to \emph{any} combination. %





\noindent\textbf{Meta-choice.} 
The assumption of conditional independence that the formulation in (\ref{eq:prob-combine}) uses is natural and makes sense in many settings. For example, during training time, we might control what feedback type we ask the human for. We might start by asking the human for demonstrations, but then move on to other types of feedback, like corrections or comparisons, to get more fine-grained information about the reward function. Since the human is only ever considering one type of feedback at a time, the conditional independence assumption makes sense.

\begin{figure*}[t]
    \centering
    \includegraphics[width=.9\textwidth]{ExperimentFigures/Metareasoning.pdf}
    \caption{\small{(Left) Environment with designated start (red circle), goal (green circle) and lava area (red tiles). The human can provide a correction (one of the green trajectories) or turn off the robot, forcing the robot to stop at the marked dot. (Middle) Belief distribution over rewards after the human provides  feedback ($\rat_0 = 10.0$). Darker indicates higher probability. The metareasoning model is able to rule out more reward functions than the naive model. (Right) When the human's metareasoning has no signal ($\rat_0 = 0$), then the metareasoning (orange) and naive model (gray) perform equally well. As $\rat_0$ increases, the advantage of the metareasoning model also increases.}}
    \label{fig:metareason_exp}
\end{figure*}

But the assumption breaks when the human has access to multiple types of feedback at once because \emph{the types of feedback the robot can interpret influence what the human does in the first place}.\footnote{We note that this adaptation by the human only applies to types of behavior that the human uses to purposefully communicate with the robot, as opposed to sources of information like initial state.} If the human intervenes and turns the robot off, that means one thing if this were the only feedback type available, and a whole different thing if, say, corrections were available too. In the latter case, we have more information - we know that the user chose to turn the robot off rather than provide a correction. %



Thus, our key insight is that the type of feedback itself leaks information about the reward, and the RRC framework gives us a recipe for formalizing this new source: %
we need to uncover the set of options the human is choosing from. %
The human has two stages of choice: the first is the choice between feedback types, i.e corrections, language, turn-off, etc. and the second is the choice within the chosen feedback type, i.e the specific correction that the human gave. Our formalism can leverage both sources of information by defining a \emph{hierarchy} of reward-rational choice.

Suppose the user has access to $n$ types of feedback with associated choice sets $\choices_1, \dots, \choices_n$, groundings $\map_1, \dots \map_n$, and Boltzmann rationalities $\beta_1, \dots, \beta_n$. For simplicity, we assume deterministic groundings. The set of choice sets $\mathscr{C}_0$ for the first-stage choice is $\{\choices_1, \dots, \choices_n\}$ The grounding $\map_0: \choices \rightarrow f_{\trajs}$ for the first stage choice maps a feedback type $\choices_i$ to the distribution of trajectories defined by the human's behavior and grounding in the second stage:
\begin{align} \label{eq:first-stage-grounding}
    \map_0(C_i)\ & =\ \pr(\traj \mid r,\, \choices_i) \nonumber  \\
    = & \sum_{\fdbk_i \in \choices_i : \map_i(\fdbk_i) = \traj} \pr(\fdbk_i \mid r,\, \choices_i) \,,
\end{align}
where, as usual, $\pr(\fdbk_i \mid r,\, \choices_i)$ is given by Equation \ref{eq:rat-choice2}. Instantiating Equation \ref{eq:rat-choice2} to model the first-stage decision as well, results in the following model for the human picking feedback type $\choices_i$:
\begin{align}
\pr(\choices_i \mid r) = \frac{\exp\big( \beta_0\cdot\mathbb{E}_{\traj \sim \map_0(\choices_i)}[r(\traj)] \big)}{\sum_{j \in [n]}\ \exp\big( \beta_0\cdot\mathbb{E}_{\traj \sim \map_0(\choices_j)}[r(\traj)] \big)} \,,
\end{align}
Finally, the probability that the human gives feedback $\fdbkch$ is
\begin{align*}
  \pr(\fdbkch \mid\reward) &  = \sum_{i} \pr(\fdbkch \mid \reward,\, \choices_i)\cdot \pr (\choices_i \mid \reward) \label{eq:meta} \\ & = \sum_{i} \Bigg ( \frac{\exp\big(\beta_i\cdot \reward(\map_i(c^*))\big)}{\sum_{\fdbk \in \choices_i}\ \exp\big(\beta_i\cdot r(\map_i(c))\big)} \\ & \cdot \frac{\exp\big( \beta_0\cdot\mathbb{E}_{\traj \sim \map_0(\choices_i)}[r(\traj)] \big)}{\sum_{j \in [n]}\ \exp\big( \beta_0\cdot\mathbb{E}_{\traj \sim \map_0(\choices_j)}[r(\traj)] \big)} \Bigg ) \,.
\end{align*}



The first-stage decision can be interpreted as the human \emph{metareasoning} over the best type of feedback. The benefit of modeling the hierarchy is that we can cleanly separate and consider noise at both the level of metareasoning ($\beta_0$) and the level of execution of feedback ($\beta_1, \dots, \beta_n$). Noise at the metareasoning level models the human's imperfection in picking the optimal type of feedback. Noise at the execution level might model the fact that the human has difficulty in physically correcting a heavy and unintuitive robot.\footnote{Although we modeled rationality with respect to the reward $r$ that the robot should optimize, we can easily extend our formalism to capture that the person might trade-off between that and their own effort -- this is especially interesting at this meta-choice level, where one type of feedback might be much more difficult and thus people might want to avoid it unless it is particularly informative.} 

We showcase the potential importance of accounting for the meta-choice in an experiment  in a gridworld setting, in which an agent navigates to a goal state while avoiding lava (Figure \ref{fig:metareason_exp}, left). The reward function is a linear combination of 2 features that encode the goal and lava. The human has access to two channels of feedback: ``off'' and corrections. We simulate the human feedback as choosing between \emph{feedback types} according to Equation \ref{eq:meta}. We manipulate three factors: 1) whether the robot is \emph{naive}, i.e. only accounts for the information \emph{within} the feedback type, or \emph{metareasons}, i.e. accounts for the other feedback types that were available but not chosen; 2) the meta-rationality parameter $\beta_0$ modeling human imperfection in selecting the optimal type of feedback; and 3) the location of the lava, so that the rational meta-choice changes from off to corrections. We measure regret over holdout environments.

Figure \ref{fig:metareason_exp} (left) depicts the possible grounded trajectories for corrections and for off. For the top, off is optimal because all corrections go through lava. For the bottom, the rational meta-choice is to correct. In both cases, we find that meta-reasoning gains the learner more information, as seen in the belief (center). For the top, where the person turns it off, the robot can be more confident that lava is bad. For the bottom, the fact that the person had the off option and did not use it informs the robot about the importance of reaching the goal. This translates into lower regret (right), especially as $\beta_0$ increases and there is more signal in the feedback type choice. 
Since this advantage depends on knowledge of the human's metarationality ($\beta_0$), in Appendix \ref{app:meta}, we also describe experiments testing the effect of misspecifying $\beta_0$.








